Resilient Constrained Learning

When deploying machine learning solutions, they must satisfy multiple requirements beyond accuracy, such as fairness, robustness, or safety. These requirements are imposed during training either implicitly, using penalties, or explicitly, using constrained optimization methods based on Lagrangian duality. Either way, specifying requirements is hindered by the presence of compromises and limited prior knowledge about the data. Furthermore, their impact on performance can often only be evaluated by actually solving the learning problem. This paper presents a constrained learning approach that adapts the requirements while simultaneously solving the learning task. To do so, it relaxes the learning constraints in a way that contemplates how much they affect the task at hand by balancing the performance gains obtained from the relaxation against a user-defined cost of that relaxation. We call this approach resilient constrained learning after the term used to describe ecological systems that adapt to disruptions by modifying their operation. We show conditions under which this balance can be achieved and introduce a practical algorithm to compute it, for which we derive approximation and generalization guarantees. We showcase the advantages of this resilient learning method in image classification tasks involving multiple potential invariances and in heterogeneous federated learning.

==> 02_problem_formulation_srm.tex <==
%!TEX root = main.tex

\blue{Alejandro Question: Do we need to talk about classification or regression explicitly?  Or can we talk about either?}
\red{Ignacio's response: It is here because of non-convex losses,the proof (lyapunov's convexity thrm) stronger assumptions in the regression case. Maybe we can just state the results and assumptions for the classification case and move reggression to the appendix for clarity.}
Consider data pairs $(\bbx, y)$ where $\bbx \in \calX \subset \reals^d$ is an input feature and $y \in \ccalY \subset \reals$ is the corresponding output. Pairs $(\bbx, y)$ are sampled according to a set of $m+1$ distributions $\ccalD_i$. Our goal is to learn a function $\phi: \ccalX \to \calY \subset\reals$ in some hypothesis space $\mathcal{F}$ that can be used to produce estimates $\phi(\bbx)$ of outputs $y$. Different from classical (unconstrained) learning, we have a set of $m+1$ bounded losses $\ell_i: \calY \times \calY \to [0, B]$ that evaluate the fitness of estimates produced by $\phi(\bbx)$ relative to outputs $y$. We then define the constrained statistical learning (CSL) problem as the program
%
\begin{prob}[P-CSL]\label{eqn_csl}
	\P ~=~  
	   &  \min_{\phi\in\ccalF}
	      && \mbE_{(\bbx, y) \sim \calD_0} 
                \Big[ \ell_0(\phi(\bbx),y)\Big], \\
	   &  \text{~s.t.}
	      && \mbE_{(\bbx, y) \sim \calD_i} 
                \Big[ \ell_i(\phi(\bbx),y)\Big] \leq 0, \quad 
                   && i = 1, \dots, m. \phantom{\Big[}
\end{prob}
%
Setting aside the constraints in \eqref{eqn_csl}; namely, if we make $m=0$, we recover the classical unconstrained statistical learning problem in which we seek the function $\phi$ that best fits the labels $y$ as dictated by the loss function $\ell_0$. The constraints $\mbE_{(\bbx, y) \sim \calD_i} [ \ell_i(\phi(\bbx),y)] \leq 0 $, with $i = 1, \dots, m$, represent desired statistical properties of function $\phi$. 
 
An important challenge in formulating meaningful \eqref{eqn_csl} problems is the specification of constraints that make the problem feasible. This is an important distinction with respect to unconstrained learning. The optimal function $\phi$ in the latter case always exists. In \eqref{eqn_csl} it may be that no function $\phi$ satisfies the given requirements. In practice, landing on satisfiable requirements may necessitate the relaxation of some constraints relative to their initial specification. Thus, in lieu of \eqref{eqn_csl} we settle for the relaxed optimization problem
%¸
\begin{prob}[P-RLX]\label{eqn_the_problem}
	\P(\bbu) ~=~  
	   &  \min_{\phi}
	      && \mbE_{(\bbx, y) \sim \calD_0} 
                \Big[ \ell_0(\phi(\bbx),y)\Big], \\
	   &  \text{~s.t.}
	      && \mbE_{(\bbx, y) \sim \calD_i} 
                \Big[ \ell_i(\phi(\bbx),y)\Big] \leq u_i, \quad 
                   && i = 1, \dots, m. \phantom{\Big[}
\end{prob}
%
In \eqref{eqn_the_problem} the constraints are relaxed to $\mbE_{(\bbx, y) \sim \calD_i} [ \ell_i(\phi(\bbx),y)] \leq  u_i$ for some nonnegative $u_i\geq 0$. When we do this, the optimal cost $\P$ changes to $\P(\bbu)$, where the variable $\bbu$ signifies all of the individual constraint relaxations $u_i$. For future reference we denote as $\phi^*(\bbx;\bbu)$ the function that solves \eqref{eqn_the_problem} and as $\phi^*(\bbx) = \phi^*(\bbx;\bbzero)$ the function that solves \eqref{eqn_csl}.

If the function class $\ccalF$ is a convex set and the losses $l_i$ are convex functions of their arguments, the perturbation function $\P(\bbu)$ is known to be convex \red{\cite{Rockafellar}.} Convexity of $\P(\bbu)$ still holds if the losses are not convex provided that the measures $\ccalD_i$ are nonatomic; see Proposition \ref{prop:pert_cvx}. In either case we can define the subdifferential of $\P(\bbu)$ as we state next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}\label{def_subdifferential} 
%
Given the convex perturbation function $\P(\bbu)$, its subdifferential $\Fre \P(\bbu)$ is the set of all  subgradients $\bbw$ such that for all $\bbv$ it holds
%
\begin{align}\label{eqn_subdifferential}
   \P(\bbv) 
      \geq \P(\bbu) 
              + \Big\langle \bbw, \bbv - \bbu \Big\rangle, 
\end{align} 
%
where $\langle \bbw, \bbv - \bbu \rangle = \sum_{i=1}^{m} \bbw_i (v_i-u_i)$ denotes the inner product of $\bbw$ and $\bbv-\bbu$. 
%
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R    %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

If the perturbation function is  differentiable at $\bbu$, then, the  derivative is a  subdifferential. In this case, the subdifferential is unique save for a set of zero measure. In general, there may be points $\bbu$ at which the perturbation function is not  differentiable. At these points the  subdifferential is not unique. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   Proposition sensitivity   %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For sufficiently large relaxations $\bbu$, Problem \eqref{eqn_the_problem} is feasible under mild conditions. The larger the relaxation, however, the less impact the constraints have on the optimal function $\phi^*(\bbx;\bbu)$. Thus, the point at issue is coming up with reasonable definitions of relaxations that are sufficiently large but not too large. The insight we adopt in this paper is to equate the marginal cost of the relaxation with the marginal cost of its effect on the optimal cost as we formally define next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}\label{def_resilient} 
%
Let $h(\bbu)$ be a  differentiable convex nondecreasing function. The resilient learning problem is the relaxed problem \eqref{eqn_the_problem} in which the constraint relaxation $\bbu^{\star}$ satisfies
%
\begin{prob}[P-RSL]\label{eqn_resilient_equilibrium}
   -\Fre h(\bbu^{\star}) \in \Fre \P(\bbu^{\star})
\end{prob} 
%
where $\Fre h(\bbu)$ is the  derivative of $h(\bbu)$. We say that $\bbu^{\star}$ is a resilient relaxation and that $\phi^{\star}(\bbx;\bbu^{\star})$ is a corresponding resilient statistical minimizer. Note that whereas we assume $h$ is  differentiable and hence its sub-differential is a singleton, the pertubation function $\P(\bbu)$ need not be differentiable. However, under certain regularity conditions $\P(\bbu^{\star})$ is indeed  diffrentiable~\cite{bonnans-perturbations}, and then satisfying the resilient equilibrium accounts for both (singleton) sets being equal.
%
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R    %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In Definition \ref{def_resilient}, the function $h(\bbu)$ measures the cost of relaxation $\bbu$. The equilibrium defined by \eqref{eqn_resilient_equilibrium} states that we seek a relaxation for which the marginal price of modifying the constraint equates its marginal benefit as measured by the change it implies in the optimal loss. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
{\footnotesize  
    \centering
    \begin{minipage}[t]{0.32\textwidth}
       \centering
       \input{figures/resilient_equilibrium_1.tex}
       Case (a)
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
       \centering
       \input{figures/resilient_equilibrium_2.tex}
       Case (b)
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
       \centering
       \input{figures/resilient_equilibrium_3.tex}
       Case (c)
    \end{minipage}
}
\caption{Resilient Equilibrium. We relax constraints to points where the marginal cost of the relaxation equals the marginal cost of its effect on the optimal cost (Definition \ref{def_resilient}). We illustrate different constraints that are increasingly easier to satisfy, i.e., from left to right the sensitivity curve shifts downwards (red curve). The resilient point corresponds to the intersection between those two curves. Constraints that are infeasible are relaxed to make them feasible (a) and constraints that are difficult to satisfy (b) are relaxed more than constraints that are easy to satisfy (c).}
\label{fig_equilibrium}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For a better understanding, consider the case of a problem with a single statistical constraint. Further, assume that we make $h(\bbu_1) = h(\bbu) = \bbu^2/2$, and that $\P(\bbu)$ is differentiable (i.e., $\Fre \P(\bbu) = \{ \partial \P(\bbu)/\partial \bbu\}$ is a singleton). We then have that the resilient relaxation is the one for which
%
\begin{align}\label{eqn_resilient_equilibrium_example}
  \bbu = - \partial \P(\bbu)/\partial \bbu.
\end{align} 
%
Figure \ref{fig_equilibrium} considers some prototypical situations that depict the intersection between the marginal cost of relaxation $\bbu$ and the marginal benefit of relaxation $ -\partial \P(\bbu)/\partial \bbu$. In all cases the negative derivative diverges at the constraint value $\bbu$ that makes the problem infeasible and decreases towards $\partial \P(\bbu)/\partial \bbu = 0$ as the constraint is relaxed. Case (a) represents a problem for which the original formulation \eqref{eqn_csl} is infeasible. The resilient equilibrium \eqref{eqn_resilient_equilibrium} produces a version of \eqref{eqn_the_problem} with a large relaxation. Case (b) illustrates a problem where \eqref{eqn_csl} is feasible but close to infeasible. The resilient equilibrium \eqref{eqn_resilient_equilibrium} produces a version of \eqref{eqn_the_problem} with a small relaxation. In case (c) \eqref{eqn_csl} is feasible and the constraint is barely active. The resilient equilibrium \eqref{eqn_resilient_equilibrium} produces a version of \eqref{eqn_the_problem} that is barely different from the original \eqref{eqn_csl}.

In general, we can think of constraints associated with larger partial derivatives $\partial \P(\bbu)/\partial \bbu_i$ as more difficult to satisfy because their relaxation results in a larger marginal decrease in the optimal value $\P(\bbu)$. The resilient equilibrium in \eqref{eqn_resilient_equilibrium} allows for a larger relaxation of these constraints. Conversely, constraints associated with smaller partial derivatives $\partial \P(\bbu)/\partial \bbu_i$ are easier to satisfy because their relaxation results in a smaller marginal increase in the optimal value $\P(\bbu)$. The resilient equilibrium in~\eqref{eqn_resilient_equilibrium} allows for a smaller relaxation of these constraints.

Note that in Figure~\ref{fig_equilibrium} $-\partial \P(\bbu)/\partial \bbu$ is decreasing, $\partial h(\bbu)/\partial \bbu$ is increasing, and the equilibrium point is unique. As shown in the next propositions, these properties follow from the convexity of the perturbation function and under strict convexity of $h$.

\begin{proposition}\label{prop:subdiff_inc} Let $\bbv, \bbu $, be two perturbation vectors such that $\bbv_i = \bbu_i$ for all $i \neq j$ and  $\bbv_j > \bbu_j$ ($\mathcal{D}_j-\text{a.e.}$ if $j>m$),
then $d\P(\bbv)_j \geq d\P(\bbu)_j$ $\forall \; {d\P(\bbv) \in \Fre \P(\bbv)}, {d\P(\bbu) \in \Fre \P(\bbu) }$.
\end{proposition}
\begin{proof}
See Appendix~\ref{pf:subdiff_inc}.
\end{proof}

Thus, the marginal benefit obtained by relaxing a constraint $-d\P(\bbu)_j$ always decreases as the constraint is relaxed. This means that the constraint of the relaxed problem is easier to satisfy. Moreover, strict convexity of $h$ implies that the resilient equilibrium point is unique, as shown in the following proposition.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   Proposition Uniqueness  %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proposition}~\label{prop:uniqueness} If $h$ is strictly convex and there exists a constraint relaxation $\bbu$ such that the resilient equilibrium~\eqref{eqn_resilient_equilibrium} is satisfied, it is unique.
\end{proposition}
\begin{proof}
See Appendix~\ref{pf:uniqueness}.
\end{proof}

In Section \ref{sec:res_learning} we introduce equivalent formulations that are important for algorithmic developments and show that, under mild conditions on the learning problem, the equilibrium in \eqref{eqn_resilient_equilibrium} indeed exists.



\red{All of the following derivations can be extended to dense constraint sets, that is, constraints on losses that are enforced almost everywhere with respect to some distribution $\ccalD_j$, leading to a semi-infinite constrained problem. In what follows, we focus on a finite constraints as in~\eqref{eqn_csl} for the sake of conciseness, and address the case of dense constraint sets in Appendix~\ref{a:pointwise}.}



\red{The function $\P(\bbu)$ is known as the perturbation function of \eqref{eqn_csl} as it describes the effect on the optimal primal value of perturbing the constraints. It is ready to verify that $\P(\bbu)$ is a decreasing function of its argument in the sense that for component-wise comparable arguments $\bbu_1 \preceq \bbu_2$ we have  $\P(\bbu_1) \geq \P(\bbu_2)$. We now give sufficient conditions under which the perturbation function $\P(\bbu)$ is convex.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   S   S   U   M   P   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{assumption} [Convex Hypothesis space]\label{ass_convexity_h_space} 
The functional hypothesis space $\mathcal{F}$ is convex.
\end{assumption}

\begin{assumption}[Convex Cost Constraint Set]\label{ass_non_convex} 
Either
\begin{enumerate}[(a)]
    \item The loss functions $\ell_i$ $i = 0,\ldots,m$ are convex.
    \item The loss functions $\ell_i$ $i = 0,\ldots,m$ are non-convex, and either
    \begin{enumerate}[(i)]
        \item (Classification) $\mathcal{Y}$ is finite, and the conditional random variables $\boldsymbol{x} \mid y$ induced by the $\mathfrak{D}_i$ is non-atomic, and $\mathcal{F}$ is decomposable.
        \item (Regression. Informally, see~\cite{non-convex}.) $\mathcal{Y}$ is compact and the losses are uniformly continuous in $y$.
    \end{enumerate}
\end{enumerate}
\end{assumption}

 Assumption~\ref{ass_convexity_h_space} requires the functional hypothesis space $\mathcal{F}$ to be convex. However, many commonly used hypothesis spaces are non-convex, most notably neural network architectures. We may thus consider the convex functional hypothesis space associated with the convex hull of a possibly non-convex parametrization. As formalized in section~\ref{sec:rl_psrm}, under certain assumptions on the hypothesis space the optimal value obtained by optimizing over the original space and over its convex hull are still close. Moreover, from a learning theoretic point of view, taking the convex hull of the hypothesis space does not affect uniform convergence rates based on Rademacher complexity~\cite{shalev2014understanding}.

Assumption~\ref{ass_non_convex}(a) holds for commonly used losses such as cross entropy and mean squared error. Allowing for non-convex losses requires introducing additional assumptions on the data distribution and hypothesis, as specified in~\ref{ass_non_convex}(b) and~\ref{ass_non_convex}(c) for classification and regression tasks, respectively. 

\begin{proposition}\label{prop:pert_cvx}
Under assumptions (\ref{ass_convexity_h_space}-\ref{ass_non_convex}) the perturbation function $P(\bbu)$ is convex.
\end{proposition}
\begin{proof}
See Appendix~\ref{pf:pert_cvx}.
\end{proof}}

==> 08_3_ERM_problem.tex <==
\section{Generalization Gap}\label{a:emp-gap}
In Appendix~\ref{a:param-gap}, we introduced a parameterized problem~\eqref{eqn_PSRM_problem} which approximates the resilient problem \eqref{eqn_resilient_equilibrium_three}. Solving problem~\eqref{eqn_PSRM_problem} requires computing expectations over distributions $\calD$, however, these distributions are not known. Instead, we have a set of sample pairs $(\bbx, y)$ randomly selected from the distribution $\calD$. Therefore, we can formulate the parameterized empirical problem
%
\begin{prob}[P-ERM]\label{eqn_ERM_problem}
	P_N^* ~=~ & \min_{\theta \in \Theta, \bbu \in \calU}&
		& \frac{1}{N}\sum_{n=1}^N \ell_0(f_\theta(\bbx_n), y_n) + h(\bbu)
	\\
	&\text{s.t.}& &   \frac{1}{N}\sum_{n=1}^N  \ell_i(f_\theta(\bbx_n), y_n) \leq u_i\text{,} \quad && i = 1, \dots, m
		\text{.}  \phantom{\Big[}
\end{prob} 
This problem is not guaranteed to be convex because of the parametrization, however, we will solve its dual problem and show that it is close to the primal resilient problem \eqref{eqn_resilient_equilibrium_three}. To this end we formulate the empirical Lagrangian
\begin{equation}
\begin{aligned}
    \calL_N(\theta, \bblam; \bbu) &= h(\bbu) + \sum_{n=1}^N \Bigg[ \frac{1}{N}\ell_0(f_\theta(\bbx_n),y_n) \\
   & +  \sum_{i=0}^m \bblam_i \bigg(\frac{1}{N}\ell_i(f_\theta(\bbx_n), y_n) - u_i\bigg)  \Bigg] \text{.}
\end{aligned} 
\end{equation}
From the Lagrangian we can formulate the dual
\begin{prob}[$D_{\epsilon,N}$]\label{eqn_dual_ERM_a}
    D_{\epsilon,N} = \max_{\bblam \geq 0} \min_{\theta \in\Theta, \bbu \in \calU} \calL_N(\theta, \bblam; \bbu) \text{.}
\end{prob}
Solving problem \eqref{eqn_dual_ERM} gives us a solution that is close to the solution of the parameterized problem.
\textbf{Assumption \ref{ass_uni_conv} [Uniform Convergence]}
 There exists $\xi(N, \delta) \geq 0$ monotonically decreasing with $N$ such that
\begin{equation*}
\left|\mathbb{E}_{\mathfrak{D}_i}\left[\ell_0\left(f_{\boldsymbol{\theta}}(\boldsymbol{x}), y\right)\right]-\frac{1}{N} \sum_{n=1}^N \ell_0\left(f_{\boldsymbol{\theta}}\left(\boldsymbol{x}_n\right), y_n\right)\right| \leq \xi(N, \delta)
\end{equation*}
for all $\boldsymbol{\theta} \in \Theta$, with probability $1-\delta$ over independent $\operatorname{draws}\left(\boldsymbol{x}_n, y_n\right) \sim \mathfrak{D}$.

\begin{proposition}\label{prop:emp_gap}
Let $D_\epsilon$ be the solution of the dual parametrized problem \eqref{eqn_dual_param_problem}, $D_{\epsilon,N}$ be the solution of the dual parametrized empirical problem \eqref{eqn_dual_ERM} if assumptions~\eqref{ass_convexity_h_space}-\eqref{ass_uni_conv} hold, then with probability $1-\gamma$ it holds that
\begin{equation}
    \vert D_\epsilon - D_{\epsilon,N} \vert \leq \xi(N),
    %V_N = 2B \sqrt{\frac{1}{N} \Bigg[ 1+ \log \Bigg(\frac{4(2N)^{d_{VC}}}{\gamma}\Bigg)\Bigg]}
\end{equation}
\end{proposition}

\begin{proof}
See Appendix~\ref{pf:emp_gap}.
\end{proof}

Finally, by combining proposition \ref{parametrization_gap} and proposition \ref{prop:emp_gap}, we can relate the dual of the empirical problem \eqref{eqn_dual_ERM} to the statistical problem \eqref{eqn_resilient_equilibrium_three}.

\begin{theorem}
Let $P$ be the solution to problem \eqref{eqn_resilient_equilibrium_three} and $D_{\epsilon,N}$ be the solution to problem \eqref{eqn_dual_ERM}. Then given assumption \ref{ass:roomy_u}, it holds with probability of $1-\gamma$ that 

\begin{equation}
    \vert P - D_{\epsilon,N} \vert \leq h(\bbu^*+L\epsilon)-h(\bbu^*) + L\epsilon + \xi(N)
\end{equation}
\end{theorem}
\begin{proof}
The proof is obtained by applying the triangle inequality to the results obtained in proposition \eqref{parametrization_gap} and \eqref{prop:emp_gap}. 
\end{proof}
%%%%%%%%%%%%%%%%%%
% I don't buy this
%%%%%%%%%%%%%%%%%%%
\iffalse
We have shown that the optimal values of \eqref{eqn_dual_ERM} and \eqref{eqn_resilient_equilibrium_three} are close, next we will prove that the corresponding primal variables are close.

\begin{theorem}[Primal bound]
    \label{thm_primal_bound}
    Let $\phi^*$ be the optimal primal variable of problem \eqref{eqn_resilient_equilibrium} and $\theta^*$ optimal primal variable of \eqref{eqn_dual_ERM}, then for any $\bbx \in \calX$ under assumptions \ref{ass_strong_convexity}, \ref{ass_losses_property}, \ref{ass:roomy_u} it holds with probability of $1-\gamma$ that
    \begin{equation} \label{eqn_primal_variable_bound}
        \vert \phi'(\bbx) - \theta^*(\bbx) \vert \leq \frac{2}{\mu} \big[ h(\bbu^*+L\epsilon)-h(\bbu^*) + L\epsilon + \xi(N) \big],
    \end{equation}
where $\bbu^*$ is the optimal perturbation, $\mu$ is the strong convexity parameter of $\ell_0$ and $\xi(N)$ as in \cite[Thm. 1]{chamon2020probably}.
\end{theorem}

\begin{proof}
Given that $\theta$ is an $\epsilon$ approximation of $\phi$ it stands to reason that any $f_\theta \in \calF$, then given that $\ell_0$ is strongly convex we have the following inequality \red{Where does this come from?}
\begin{equation}
    \vert f_{\theta^*}(\bbx) - \phi^*(\bbx) \leq \frac{2}{\mu} (D_{\epsilon,N} - P^*) \leq \frac{2}{\mu} \big[ h(\bbu^*+L\epsilon)-h(\bbu^*) + L\epsilon + \xi(N)\big]
\end{equation}
this concludes the proof.
\end{proof}
\fi


==> 08_5_CSLbounds.tex <==
\section{Comparison with Constrained learning Bounds.}~\label{a:bound-comparison}
For a fixed relaxation $\bbu^{\star}$, existing duality gap bounds from constrained learning theory~\cite{chamon2020probably} also hold under the stronger assumption that the problem with constraints tightened by $L\epsilon$ is also strictly feasible. Explicitly, if we fix $\bbu=\bbu^{\star}$ on~\eqref{eqn_the_problem}, from~\cite{chamon2020probably} we have that the duality gap is bounded by
$$
\left(P(\bbu)-D_{\epsilon}(\bbu)\right) \leq \| \bblam^* \|_1  L\epsilon + L\epsilon := d^{\text{csl}}_{\text{gap}}, 
$$
where $\bblam_i^{\star}$ are optimal dual variables of the perturbed problem.
However, due to the convexity of $h$, the duality gap bound of the resilient problem from proposition~\eqref{parametrization_gap} $D_\epsilon - P_{res} \leq h(\bbu^{\star}+L\epsilon) -h(\bbu^{\star}) + L\epsilon :=d^{\text{rsl}}_{\text{gap}}$  is tighter, as detailed in the next proposition.
\begin{proposition}\label{cor:gap-vs-csl}
Let $d^{\text{rsl}}_{\text{gap}}$ and $d^{\text{csl}}_{\text{gap}}$ be the duality gap bounds for the resilient and constrained learning problem  defined above, it holds
\begin{equation}
    d^{\text{rsl}}_{\text{gap}}\leq d^{\text{csl}}_{\text{gap}}
\end{equation}
Additionally, if $h$ is strictly convex with parameter $\mu>0$, it holds:
\begin{equation}
     d^{\text{csl}}_{\text{gap}} - d^{\text{rsl}}_{\text{gap}}  \geq \mu (L\epsilon)^2
\end{equation}
\end{proposition}
\begin{proof}
From the resilient equilibrium condition~\eqref{eqn_resilient_equilibrium_two} we have that
\begin{equation}\label{eqn_dh_bblam}
\frac{\partial h (\bbu + L\epsilon)}{\partial \bbu} = \bblam^*,
\end{equation}
where $\bblam^{\star}$ denotes the optimal dual variables of the perturbed problem.

The difference between the duality gap bounds is
\begin{align}
d^{\text{csl}}_{\text{gap}} - d^{\text{rsl}}_{\text{gap}}  = \| \bblam^*\|_1 L\epsilon -(h(\bbu+L\epsilon)-h(\bbu))
\end{align}
Substituting~\eqref{eqn_dh_bblam} we get
\begin{align}\label{eqn_diff_dual_gap}
d^{\text{csl}}_{\text{gap}} - d^{\text{rsl}}_{\text{gap}}  =  \left\|\frac{\partial h (\bbu+L\epsilon)}{\partial \bbu}\right\|_1 + h(\bbu) - h(\bbu+L\epsilon).
\end{align}
First, the convexity of $h$~(Assumption \ref{ass_convexity_h_space}) implies the following first order condition is satisfied
\begin{equation}\label{eqn_first_order}
h(\bbu) \geq h(\bbu+L\epsilon) - \left\|\frac{\partial h (\bbu+L\epsilon)}{\partial \bbu}\right\|_1 L\epsilon,
\end{equation}
Rearranging terms we get
\begin{equation}
    0 \leq  \left\|\frac{\partial h (\bbu+L\epsilon)}{\partial \bbu}\right\|_1 L\epsilon + h(\bbu) - h(\bbu+L\epsilon) = d^{\text{csl}}_{\text{gap}} - d^{\text{rsl}}_{\text{gap}}, 
\end{equation}
Proving the first inequality.

Now if h is strongly convex, it satisfies
\begin{equation}\label{eqn_second_order}
h(u) \geq h(u+L\epsilon) - \left\|\frac{\partial h (u+L\epsilon)}{\partial u}\right\|_1 L\epsilon + \mu (L\epsilon)^2
\end{equation}
Again, rearranging terms and substituting in~\eqref{eqn_diff_dual_gap}  yields the desired inequality.
\end{proof}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
%\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
%\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

